Large pseudoscalar Yukawa couplings in the complex 3HDM

As LHC's Run3 unfolds, we peer deeper into the couplings of the 125GeV Higgs ($h_{125}$) and also test for extra scalars. Even before such extra scalars are found, one can probe them by using the fact that theories with multiple Higgs doublets allow for substantial deviations of the couplings of $h_{125}$ from their SM values. Indeed, the observed couplings already place stringent limits on such theories. We investigate the curious possibility that $h_{125}$ couples to the top quark mostly as a scalar, while it couples to the bottom quark mostly as a pseudoscalar. This possibility was allowed by 2017 data for the so-called C2HDM; a two Higgs doublet model with a single source of explicit CP violation. It was shown recently that this possibility disappears when using the full experimental data of 2024. Here we discuss a three Higgs doublet with explicit CP violation (C3HDM), and show that the curious CP-even/CP-odd $t$/$b$ possibility is partly resuscitated, prompting further experimental exploration of this prospect.

==> Makefile <==
FILENAME=C3HDM
LATEX = pdflatex
BIBTEX = bibtex
PDFTOPS = pdftops
AR = acroread
GV = gv
EV = evince
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

PSFILE = C3HDM.ps 
PDFFILE = C3HDM.pdf

COPY = if test -r C3HDM.toc; then cp C3HDM.toc C3HDM.toc.bak; fi 
RM = /bin/rm -f


CLEAN=rm -f C3HDM.aux C3HDM.log C3HDM.dvi C3HDM.toc C3HDM.out C3HDM.blg C3HDM.mtc C3HDM.mtc1 C3HDM.rel C3HDM.vrb C3HDM.end C3HDM.spl C3HDM.synctex.gz C3HDMNotes.bib *~ \#* *.aux

WARNING=egrep -i "(Reference|Citation).*undefined" C3HDM.log ; true

main:	C3HDM.tex pdf

pdf:	$(PDFFILE)
	$(WARNING)  

all:	$(PDFFILE) $(PSFILE)
	$(WARNING)  

ps:	$(PSFILE) 
	$(WARNING)

gv:	$(PSFILE)
	$(GV) $(PSFILE) &
	$(WARNING)

	$(WARNING)

ev:	$(PDFFILE)
	$(EV) $(PDFFILE) &

ar:	$(PDFFILE)
	$(AR) $(PDFFILE) &

%.pdf:	%.tex
	$(COPY);$(LATEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ;true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	if [  'cmp -s $*.toc $*.toc.bak'  ]; then $(LATEX) $< ; fi
	$(RM) $*.toc.bak

%.ps:	%.pdf
	$(PDFTOPS) $<

clean:	
	$(CLEAN)

realclean: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).pdf $(FILENAME).bbl
	$(RM) $(FILENAME).lof $(FILENAME).lot $(FILENAME).rel

cleanps: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).bbl

complete:$(PDFFILE)
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).bbl



